Random Hash Code Generation for Cancelable Fingerprint Templates using Vector Permutation and Shift-order Process

Cancelable biometric techniques have been used to prevent the compromise of biometric data by generating and using their corresponding cancelable templates for user authentication. However, the non-invertible distance preserving transformation methods employed in various schemes are often vulnerable to information leakage since matching is performed in the transformed domain. In this paper, we propose a non-invertible distance preserving scheme based on vector permutation and shift-order process. First, the dimension of feature vectors is reduced using kernelized principle component analysis (KPCA) prior to randomly permuting the extracted vector features. A shift-order process is then applied to the generated features in order to achieve non-invertibility and combat similarity-based attacks. The generated hash codes are resilient to different security and privacy attacks whilst fulfilling the major revocability and unlinkability requirements. Experimental evaluation conducted on 6 datasets of FVC2002 and FVC2004 reveals a high-performance accuracy of the proposed scheme better than other existing state-of-the-art schemes.

==> egbib.tex <==
@article{RN24,
   author = {Cappelli, Raffaele and Ferrara, Matteo and Maltoni, Davide},
   title = {Minutia Cylinder-Code: A New Representation and Matching Technique for Fingerprint Recognition},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   volume = {32},
   number = {12},
   pages = {2128-2141},
   ISSN = {0162-8828},
   DOI = {10.1109/tpami.2010.52},
   url = {<Go to ISI>://WOS:000283558700002},
   year = {2010},
   type = {Journal Article}
}

@article{RN25,
   author = {Chen, Yanzhi and Wo, Yan and Xie, Renjie and Wu, Chudan and Han, Guoqiang},
   title = {Deep Secure Quantization: On secure biometric hashing against similarity-based attacks},
   journal = {Signal Processing},
   volume = {154},
   pages = {314-323},
   ISSN = {0165-1684},
   DOI = {10.1016/j.sigpro.2018.09.013},
   url = {<Go to ISI>://WOS:000448096000030},
   year = {2019},
   type = {Journal Article}
}

@article{RN26,
   author = {Feng, Yi C. and Lim, Meng-Hui and Yuen, Pong C.},
   title = {Masquerade attack on transform-based binary-template protection based on perceptron learning},
   journal = {Pattern Recognition},
   volume = {47},
   number = {9},
   pages = {3019-3033},
   ISSN = {0031-3203},
   DOI = {10.1016/j.patcog.2014.03.003},
   url = {<Go to ISI>://WOS:000336872000018},
   year = {2014},
   type = {Journal Article}
}

@article{RN27,
   author = {Ferrara, Matteo and Maltoni, Davide and Cappelli, Raffaele},
   title = {Noninvertible Minutia Cylinder-Code Representation},
   journal = {IEEE Transactions on Information Forensics and Security},
   volume = {7},
   number = {6},
   pages = {1727-1737},
   ISSN = {1556-6013},
   DOI = {10.1109/tifs.2012.2215326},
   url = {<Go to ISI>://WOS:000311702600006},
   year = {2012},
   type = {Journal Article}
}

@article{RN30,
   author = {Gomez-Barrero, Marta and Galbally, Javier and Rathgeb, Christian. and Busch, Christopher},
   title = {General Framework to Evaluate Unlinkability in Biometric Template Protection Systems},
   journal = {IEEE Transactions on Information Forensics and Security},
   volume = {13},
   number = {6},
   pages = {1406-1420},
   ISSN = {1556-6013},
   DOI = {10.1109/tifs.2017.2788000},
   url = {<Go to ISI>://WOS:000424738000005},
   year = {2018},
   type = {Journal Article}
}

@article{RN32,
   author = {Jin, Zhe and Lim, Meng-Hui and Teoh, Andrew Beng Jin and Goi, Bok-Min},
   title = {A non-invertible Randomized Graph-based Hamming Embedding for generating cancelable fingerprint template},
   journal = {Pattern Recognition Letters},
   volume = {42},
   pages = {137-147},
   ISSN = {0167-8655},
   DOI = {10.1016/j.patrec.2014.02.011},
   url = {<Go to ISI>://WOS:000333451300018},
   year = {2014},
   type = {Journal Article}
}

@article{RN33,
   author = {Jin, Zhe and Lim, Meng-Hui and Teoh, Andrew Beng Jin and Goi, Bok-Min and Tay, Yong Haur},
   title = {Generating Fixed-Length Representation From Minutiae Using Kernel Methods for Fingerprint Authentication},
   journal = {IEEE Transactions on Systems Man Cybernetics-Systems},
   volume = {46},
   number = {10},
   pages = {1415-1428},
   ISSN = {2168-2216},
   DOI = {10.1109/tsmc.2015.2499725},
   url = {<Go to ISI>://WOS:000384313400008},
   year = {2016},
   type = {Journal Article}
}

@article{RN34,
   author = {Kho, Jun Beom and Kim, Jaihie and Kim, Ig-Jae and Teoh, Andrew Beng Jin},
   title = {Cancelable fingerprint template design with randomized non-negative least squares},
   journal = {Pattern Recognition},
   volume = {91},
   pages = {245-260},
   ISSN = {0031-3203},
   DOI = {10.1016/j.patcog.2019.01.039},
   url = {<Go to ISI>://WOS:000466250400020},
   year = {2019},
   type = {Journal Article}
}

@article{RN35,
   author = {Lee, Chulhan and Choi, Jeung-Yoon and Toh, Kar-Ann and Lee, Sangyoun and Kim, Jaihie},
   title = {Alignment-free cancelable fingerprint templates based on local minutiae information},
   journal = {IEEE Transactions on Systems Man and Cybernetics Part B-Cybernetics},
   volume = {37},
   number = {4},
   pages = {980-992},
   ISSN = {1083-4419},
   DOI = {10.1109/tsmcb.2007.896999},
   url = {<Go to ISI>://WOS:000247833000018},
   year = {2007},
   type = {Journal Article}
}

@article{RN36,
   author = {Manisha, Kumar and Kumar, Nitin},
   title = {Cancelable Biometrics: a comprehensive survey},
   journal = {Artificial Intelligence Review},
   volume = {53},
   number = {5},
   pages = {3403-3446},
   ISSN = {0269-2821},
   DOI = {10.1007/s10462-019-09767-8},
   url = {<Go to ISI>://WOS:000534130800010},
   year = {2020},
   type = {Journal Article}
}

@article{RN45,
   author = {Murakami, Takao and Fujita, Ryo and Ohki, Tetsushi and Kaga, Yosuke and Fujio, Masakazu and Takahashi, Kenta},
   title = {Cancelable Permutation-Based Indexing for Secure and Efficient Biometric Identification},
   journal = {IEEE Access},
   volume = {7},
   pages = {45563-45582},
   ISSN = {2169-3536},
   DOI = {10.1109/access.2019.2908456},
   url = {<Go to ISI>://WOS:000465477300001},
   year = {2019},
   type = {Journal Article}
}

@article{RN37,
   author = {Patel, Vishal M. and Ratha, Nalini K. and Chellappa, Rama},
   title = {Cancelable Biometrics A review},
   journal = {IEEE Signal Processing Magazine},
   volume = {32},
   number = {5},
   pages = {54-65},
   ISSN = {1053-5888},
   DOI = {10.1109/msp.2015.2434151},
   url = {<Go to ISI>://WOS:000359585200010},
   year = {2015},
   type = {Journal Article}
}

@article{RN38,
   author = {Ratha, Nalini K. and Chikkerur, Sharat and Connell, Jonathan H. and Bolle, Ruud M.},
   title = {Generating cancelable fingerprint templates},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   volume = {29},
   number = {4},
   pages = {561-572},
   ISSN = {0162-8828},
   DOI = {10.1109/tpami.2007.1004},
   url = {<Go to ISI>://WOS:000244855600005},
   year = {2007},
   type = {Journal Article}
}

@article{RN39,
   author = {Shahzad, Muhammad and Wang, Song and Deng, Guang and Yang, Wencheng},
   title = {Alignment-free cancelable fingerprint templates with dual protection},
   journal = {Pattern Recognition},
   volume = {111},
   ISSN = {0031-3203},
   DOI = {10.1016/j.patcog.2020.107735},
   url = {<Go to ISI>://WOS:000601158800004},
   year = {2021},
   type = {Journal Article}
}

@article{RN40,
   author = {Trivedi, Amit Kumar and Thounaojam, Dalton Meitei and Pal, Shyamosree},
   title = {Non-Invertible cancellable fingerprint template for fingerprint biometric},
   journal = {Computers \& Security},
   volume = {90},
   ISSN = {0167-4048},
   DOI = {10.1016/j.cose.2019.101690},
   url = {<Go to ISI>://WOS:000520609000006},
   year = {2020},
   type = {Journal Article}
}

@article{RN41,
   author = {Wang, Song and Deng, Guang and Hu, Jiankun},
   title = {A partial Hadamard transform approach to the design of cancelable fingerprint templates containing binary biometric representations},
   journal = {Pattern Recognition},
   volume = {61},
   pages = {447-458},
   ISSN = {0031-3203},
   DOI = {10.1016/j.patcog.2016.08.017},
   url = {<Go to ISI>://WOS:000385899400034},
   year = {2017},
   type = {Journal Article}
}

@article{RN42,
   author = {Wang, Song and Yang, Wencheng and Hu, Jiankun},
   title = {Design of Alignment-Free Cancelable Fingerprint Templates with Zoned Minutia Pairs},
   journal = {Pattern Recognition},
   volume = {66},
   pages = {295-301},
   ISSN = {0031-3203},
   DOI = {10.1016/j.patcog.2017.01.019},
   url = {<Go to ISI>://WOS:000397371800027},
   year = {2017},
   type = {Journal Article}
}

@article{RN43,
   author = {Yang, Wencheng and Wang, Song and Hu, Jiankun and Zheng, Guanglou and Valli, Craig},
   title = {Security and Accuracy of Fingerprint-Based Biometrics: A Review},
   journal = {Symmetry-Basel},
   volume = {11},
   number = {2},
   DOI = {10.3390/sym11020141},
   url = {<Go to ISI>://WOS:000460767300019},
   year = {2019},
   type = {Journal Article}
}

@article{dong2020,
   author = {Dong, Xingbo and Jin, Zhe and Andrew, Beng Jin Teoh and Tistarelli, Massimo and Wong, KokSheik},
   title = {On the Security Risk of Cancelable Biometrics},
   journal = {In arXiv preprint},
   volume = {arXiv:1910.07770v3},
   number = {},
   DOI = {},
   url = {arXiv:1910.07770v3},
   year = {2020},
   type = {Journal Article}
}

@article{charikar2002,
   author = {Charikar, Moses S.},
   title = {Similarity estimation techniques from rounding algorithms},
   journal = {In Proc. ACM Symp. Theory Computation},
   pages = {308-388},
   year = {2002},
   type = {Conefernce Article}
}
‏ 
@article{scholkopf1998,
   author = {Scholkopf, B and Smola, A and Muller, KR},
   title = {Nonlinear component analysis as a kernel eigenvalue problem},
   journal = {Neural Computation},
   volume = {10},
   number = {5},
   pages = {1299-1319},
   year = {1998},
   type = {Journal Article}
}

@article{nalini2001,
  author={Nalini K., Ratha and Jonathan, H. Connell and Ruud, M. Bolle}, 
  title={Enhancing security and privacy in biometrics-based authentication systems},
  journal={IBM Systems Journal}, 
  year={2001},
  volume={40},
  number={3},
  pages={614-634},
  type = {Journal Article}
}

@article{jain2008,
   author = {Jain, Anil K. and Nandakumar, Karthik and Nagar, Abhishek},
   title = {Biometric template security},
   journal = {Eurasip Journal on Advances in Signal Processing},
   ISSN = {1687-6180},
   year = {2008},
   type = {Journal Article}
}

@article{nandakumar2015,
   author = {Nandakumar, Karthik and Jain, Anil K.},
   title = {Biometric Template Protection Bridging the performance gap between theory and practice},
   journal = {IEEE Signal Processing Magazine},
   volume = {32},
   number = {5},
   pages = {88-100},
   ISSN = {1053-5888},
   DOI = {10.1109/msp.2015.2427849},
   year = {2015},
   type = {Journal Article}
}

@article{jain2016,
   author = {Jain, Anil K. and Nandakumar, Karthik and Ross, Arun},
   title = {50 years of biometric research: Accomplishments, challenges, and opportunities},
   journal = {Pattern Recognition Letters},
   volume = {79},
   pages = {80-105},
   ISSN = {0167-8655},
   DOI = {10.1016/j.patrec.2015.12.013},
   year = {2016},
   type = {Journal Article}
}  

@article{RN28,
   author = {Ghammam, Loubna and Karabina, Koray and Lacharme, Patrick and Thiry-Atighehchi, Kevin},
   title = {A Cryptanalysis of Two Cancelable Biometric Schemes Based on Index-of-Max Hashing},
   journal = {IEEE Transactions on Information Forensics and Security},
   volume = {15},
   pages = {2869-2880},
   ISSN = {1556-6013},
   DOI = {10.1109/tifs.2020.2977533},
   url = {<Go to ISI>://WOS:000524505300001},
   year = {2020},
   type = {Journal Article}
}
  
@article{RN29,
   author = {Gomez-Barrero, Marta and Galbally, Javier},
   title = {Reversing the irreversible: A survey on inverse biometrics},
   journal = {Computers \& Security},
   volume = {90},
   ISSN = {0167-4048},
   DOI = {10.1016/j.cose.2019.101700},
   url = {<Go to ISI>://WOS:000520609000010},
   year = {2020},
   type = {Journal Article}
}  

@article{zjin2018,
   author = {Jin, Zhe and Hwang, Jung Yeon and Lai, Yen-Lung and Kim, Soohyung and Teoh, Andrew Beng Jin},
   title = {Ranking-Based Locality Sensitive Hashing-Enabled Cancelable Biometrics: Index-of-Max Hashing},
   journal = {IEEE Transactions on Information Forensics and Security},
   volume = {13},
   number = {2},
   pages = {393-407},
   ISSN = {1556-6013},
   DOI = {10.1109/tifs.2017.2753172},
   url = {<Go to ISI>://WOS:000417894200011},
   year = {2018},
   type = {Journal Article}
}  
  
@article{jin2014,
   author = {Jin, Zhe and Goi, Bok-Min and Teoh, Andrew and Tay, Yong Haur},
   title = {A two-dimensional random projected minutiae vicinity decomposition-based cancellable fingerprint template},
   journal = {Security and Communication Networks},
   volume = {7},
   number = {11},
   pages = {1691-1701},
   ISSN = {1939-0114},
   DOI = {10.1002/sec.865},
   year = {2014},
   type = {Journal Article}
}

@INPROCEEDINGS{andrew2006,  
author={Andrew, Teoh Beng Jin},  
booktitle={2006 Conference on Computer Vision and Pattern Recognition Workshop (CVPRW'06)},   
title={Cancellable Biometrics and Multispace Random Projections},   year={2006},  volume={},  
number={},  
pages={164-164},  
doi={10.1109/CVPRW.2006.49}
}

@ARTICLE{helala2018,
  author={Helala, Alshehri and Muhammad Hussain and Hatim, A. Aboalsamh and Mansour, A. Al Zuair},
  journal={IEEE Access}, 
  title={Cross-Sensor Fingerprint Matching Method Based on Orientation, Gradient, and Gabor-HoG Descriptors With Score Level Fusion}, 
  year={2018},
  volume={6},
  number={},
  pages={28951-28968},
  doi={10.1109/ACCESS.2018.2840330}
}

@ARTICLE{alessandra2013,  
  author={Alessandra A., Paulino and Jianjiang, Feng and Anil, K. Jain},  
  journal={IEEE Transactions on Information Forensics and Security},   
  title={Latent Fingerprint Matching Using Descriptor-Based Hough Transform},   
  year={2013},  
  volume={8},  
  number={1},  
  pages={31-45},  
  doi={10.1109/TIFS.2012.2223678}
}

@ARTICLE{sani2020,
  author={Sani M., Abdullahi and Hongxia, Wang and Tao, Li},
  journal={IEEE Transactions on Information Forensics and Security}, 
  title={Fractal Coding-Based Robust and Alignment-Free Fingerprint Image Hashing}, 
  year={2020},
  volume={15},
  number={},
  pages={2587-2601},
  doi={10.1109/TIFS.2020.2971142}
}

@INPROCEEDINGS{narishige2015,  
  author={Narishige, Abe and Shigefumi, Yamada and Takashi Shinzaki},  
  booktitle={2015 IEEE 7th International Conference on Biometrics Theory, Applications and Systems (BTAS)},   
  title={Irreversible fingerprint template using Minutiae Relation Code with Bloom Filter},   
  year={2015},  
  volume={},  
  number={},  
  pages={1-7},  
  doi={10.1109/BTAS.2015.7358770}
}

@INPROCEEDINGS{patrick2013,  
  author={Patrick, Lacharme and Estelle Cherrier and Christophe Rosenberger},     
  booktitle={2013 International Conference on Security and Cryptography (SECRYPT)},   
  title={Preimage attack on BioHashing},   
  year={2013},  
  volume={},  
  number={},  
  pages={1-8},  doi={}
}

@InProceedings{wang2021,
    author    = {Wang, Hanrui and Dong, Xingbo and Jin, Zhe and Teoh, Andrew Beng Jin and Tistarelli, Massimo},
    title     = {Interpretable Security Analysis of Cancellable Biometrics Using Constrained-Optimized Similarity-Based Attack},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV) Workshops},
    month     = {January},
    year      = {2021},
    pages     = {70-77}
}

@INPROCEEDINGS{kiran2018,
  author={Kiran B., Raja and Ramachandra, Raghavendra and Christoph, Busch},
  booktitle={21st International Conference on Information Fusion (FUSION)}, 
  title={Towards Protected and Cancelable Multi-Spectral Face Templates Using Feature Fusion and Kernalized Hashing}, 
  year={2018},
  volume={},
  number={},
  pages={2098-2106},
  doi={10.23919/ICIF.2018.8455809}
}
